On the Impossibility of Specification Testing of Interference Models Based on Exposure Mappings

Researchers use interference models based on exposure mappings to facilitate estimation of causal effects in randomized experiments with interference. To test the veracity of such models, researchers can use specification tests that aim to detect departures from the stipulated model. However, existing tests suffer from poor power and are often unable to detect important model violations. The main result in this paper is to show that the specification testing problem for exposure mapping models is inherently difficult, and the poor power of existing tests is inescapable. In particular, the worst-case Type I and Type II error rates must sum to one for any specification test of such models, ruling out the existence of a uniformly consistent test. This is the worst-case overall error rate achieved by a naive test that discards all data and arbitrarily rejects the null at random; the testing problem is in this sense impossible. This negative result holds true for all exposure mappings, all sample sizes, for uniformly bounded outcomes, and for alternatives that are maximally separated from the null. While some tests can detect some type of departures from the null model, there will always be relevant departures from the null that are undetectable. Informative specification tests must therefore restrict the alternative model against which they seek to attain power for, beyond the restrictions imposed by the exposure mappings alone. We illustrate this by providing a uniformly consistent test for differentiating no-interference from a network-linear-in-means model.

==> tex/preliminaries.tex <==
\section{Design-Based Framework for Network Interference} \label{sec:framework}

\subsection{Preliminary Definitions} \label{sec:preliminaries}

We consider an randomized experiment with $n$ subjects.
The experimenter selects an intervention $\zv$ from a set of interventions $\allinterventions$.
Commonly, 


 the experimenter assigns a binary treatment $z_i \in \setb{0,1}$ to each subject.
The \emph{intervention} is the entire treatment assignment vector $\zv = \paren{z_1, z_2, \dots z_n}$ and we denote the set of all interventions as $\allinterventions = \setb{0,1}^n$.
The \emph{experimental design} is the randomized treatment assignment mechanism chosen by the experimenter.
Formally, an experimental design is a probability measure $\design$ on the measurable space of interventions $(\allinterventions, \events)$ where $\events = 2^\allinterventions$.

Each subject $i \in [n]$ has an associated \emph{potential outcome function} $y_i: \allinterventions \to \Reals$ which describes all outcomes which we may potential observe in the experiment.
Note that a subject's potential outcome can depend on the treatment assigned to any other subject, i.e. we are allowing for the presence of interference.
We consider explicit models on potential outcome functions, including those that describe the interference, in the next section.
For notational convenience, we collect the $n$ individual potential outcome functions into a single \emph{entire potential outcome function} $\yv : \allinterventions \to \Reals^n$ given as
\[
\yv(\zv) = \paren{ y_1(\zv), y_2(\zv), \dots y_n(\zv) } \enspace.
\]

Experimenters often have a particular network from which they will construct a model of interference.
Throughout the paper, we let $G = (V,E)$ be an undirected graph whose vertices $V$ are the experimental subjects $\setb{1, 2, \dots n}$ and whose edge set is $E$.
We denote the \emph{neighborhood} of unit $i$ as $\neighi = \setb{ j : (i,j) \in E }$ and the \emph{degree} of unit $i$ as $\degree{i} = \abs{ \neighi }$.
The \emph{extended neighborhood} is denoted $\eneighi = \neighi \cup \setb{i}$.

We adopt the \emph{design-based} framework where subjects, their potential outcome functions, and the network $G$ are all taken to be deterministic.
In this framework, treatment assignment $\zv$ is the sole source of randomness and serves as the basis for all statistical inference.

The fundamental problem of causal inference is that while the experimenter might wish to know some structural aspects of the potential outcome functions $y_1, y_2, \dots y_n$, they are only able to observe one evaluation $y_1(\zv), y_2(\zv), \dots y_n(\zv)$ under the chosen intervention $\zv \in \allinterventions$.
In cases where the experimenter seeks to investigate a contrastive treatment effect $\tau = (1/n) \sum_{i=1}^n y_i( \zv_{i,1} ) - y_i(\zv_{i,0})$ defined with respect to contrasting interventions $\zv_{i,1}$ and $\zv_{i,0}$, precise estimates can be obtained under suitable assumptions on the potential outcome functions, i.e. correctly specified interference models.
We do not investigate the estimator of treatment effects in this paper; instead, we study the problem of using experimentally collected data to determine whether the interference model is indeed correctly specified.
We formulate this goal in the next two sections.

\subsection{Exposure Mapping Models} \label{sec:outcome-models}

Experimenters encode their assumptions about the nature of network interference thru the specification of a model on the potential outcome functions.
For each subject $i \in [n]$, the experimenter will posit that $y_i \in \modelspace_i$ for a linear space of functions $\modelspace_i$.
We define $\modelspace = \modelspace_1 \times \modelspace_2 \times \dots \times \modelspace_n$ so that the correctly specified assumption may be stated concisely as $\yv \in \modelspace$.
While a variety of model spaces are possible in design-based inference, the most popular model is the exposure mapping model of \citet{Aronow2017Estimating}.

Before formally defining the class of exposure mapping models, we develop some notation for partitions.
Let $\rho$ be a partition of the interventions $\allinterventions$, i.e. $\rho = \setb{ R_1 \dots R_m }$ where $R_k \subseteq \allinterventions$, $R_l \cap R_k = \emptyset$ for $l \neq k$ and $\cup_{k=1}^m R_k = \allinterventions$.
In an abuse of notation, we will also use $\rho$ to denote the function which maps an intervention $\zv$ to the subset $R \in \rho$ to which it belongs, i.e. if $\zv \in R_k$ then we will write $\rho(\zv) = R_k$.
Given partitions $\rho$ and $\alpha$ of $\allinterventions$, we say that $\alpha$ is a \emph{refinement} of $\rho$ if for each $A \in \alpha$, there exists $R \in \rho$ such that $A \subseteq R$.
In another slight abuse of notation, we use $\rho$ to also denote the mapping from a set $A$ in the finer partition to its corresponding set $R$ in the coarse partition, i.e. $\rho(A) = R$.

An exposure mapping model is defined by specifying a sequence of unit-specific partitions $\rho_1, \rho_2, \dots \rho_n$ , which we collect as $\rv = (\rho_1, \rho_2, \dots, \rho_n)$.

\begin{definition} \label{def:exposure-mapping-model}
	An \emph{exposure mapping model} $\modelspace_{\rv}$ determined by a sequence of partitions $\rv = (\rho_1, \rho_2, \dots, \rho_n)$ as defined as
	\[
	\modelspace_{\rv} = \setb{ \yv : \allinterventions \to \Reals^n : y_i(\zv) = y_i(\zv') \text{ for all } i \in [n] \text{ and } \zv, \zv' \in \allinterventions \text{ with } \rho_i(\zv) = \rho_i(\zv')
	}
	\enspace.
	\]
\end{definition}

The key idea behind the exposure mapping model is simple: for each subject, the experimenter specifies a partition $\rho = \setb{R_1, \dots R_m}$ of the intervention set $\allinterventions$ and assumes that the potential outcome function $y_i$ is constant on each group $R_k$.
Each of these groups $R_1 \dots R_k$ is referred to as an \emph{exposure} and the number of exposures for a given unit is typically small.
In this way, each potential outcome function depends on the entire intervention vector $\zv$ but only through the received exposure $\rho_i(\zv)$.
Thus, an exposure mapping model serves to reduce the complexity of potential outcome functions while still capturing the presumed structure of network interference.

The following corollary shows that every potential outcome function in the exposure mapping model may be written using coefficients which correspond to elements in its partition.

\begin{corollary} \label{corollary:equivalent-exposure-map-def}
	Exposure mapping models may be equivalently characterized as follows:
	 $\yv \in \modelspace_{\rv}$ if there exists real coefficients $\alpha_{i,R}$ for each $i \in [n]$ and $R \in \rho_i$ such that
	\[
	y_i(\zv) = \sum_{R \in \rho_i} \alpha_{i,R} \indicator{\zv \in R}
	\enspace.
	\]
\end{corollary}

It is often convenient to work with these coefficients, as they represent the value that the potential outcome function can take on an element in the partition, i.e. if $R \in \rho_i$ is a partition element containing assignment $\zv$, then $\yv_i(\zv) = \alpha_{i,R}$.
To illustrate the expressivity of exposure mapping models, we provide several examples below:

\begin{itemize}
	\item \textbf{No Treatment Effect}
	Consider the model $\modelspace$ where each potential outcome function is constant, i.e. $y_i(\zv) = \alpha_{i}$ for each $i \in [n]$.
	In this case, each unit's partition is the entire intervention set, i.e. $\rho_i = \allinterventions$.
	These models arise commonly as null hypotheses in Fisher-style permutation tests.
	
	\item \textbf{No Interference}
	The most common model in causal inference is the Stable Unit Treatment Value Assumption (STUVA) model with binary treatments.
	In this case, $\yv \in \modelspace$ if $y_i(\zv) = \alpha_{i,1} \indicator{z_i = 1} + \alpha_{i,0} \indicator{z_i = 0}$.
	To see that this is an exposure mapping model, observe that we may select each unit's partition to be $\rho_i = \setb{R_0, R_1}$ where $R_k = \setb{ \zv \in \allinterventions : z_k = k }$.
	
	\item \textbf{Simple Interference}
	We provide a simple interference model which has four exposures to account for direct and indirect treatment and is commonly used in field experiments \citep{Paluck2016Changing, Aronow2017Estimating}.
	Intuitively, the exposure depends on whether a unit has received treatment and whether any of their peers have received treatment.
	Formally, the partition is given as $\rho_i = \setb{ R_{0,0}, R_{0,1}, R_{1,0}, R_{1,1} }$ where
	\[
	R_{k,1} = \setb{ z_i = k \text{ and } \exists j \in \neighi : z_j = 1 }
	\quadand
	R_{k,0} = \setb{ z_i = k \text{ and } z_j = 0 \ \forall \ j \in \neighi }
	\enspace.
	\]
	While this simple exposure mapping model accounts of interference, it is somewhat restricted. For example, the model does not make a distinction between 1 neighbor receiving treatment and all neighbors receiving treatment.
	
	\item \textbf{Arbitrary Neighborhood Interference}
	A more complex exposure mapping model is one in which each subject's potential outcome function is an arbitrary function of the treatments given to itself and its neighbors.
	Such a model can be realized thru the partition $\rho_i = \setb{ R_{\vec{s}} : \vec{s} \in \setb{0,1}^{\eneighi} }$, where $R_{\vec{s}}$ collects the interventions $\zv$ where $z_j = s_j$ for each $j \in \eneighi$.
	Here, the number of exposures is $2^{\degreei + 1}$ for each unit $i \in [n]$.
\end{itemize}

We would like to understand when one exposure mapping model is a sub-model of another.
The following proposition shows that this is characterized by the notion of partition refinement.

\begin{proposition} \label{prop:submodel-refinement}
	For exposure mapping models, $\modelspace_{\rv} \subseteq \modelspace_{\av}$ if and only if $\alpha_i$ is a refinement of $\rho_i$ for each $i \in [n]$.
\end{proposition}

The exposure mapping models discussed above were presented in a nested order.
In particular, the constant outcome model is a submodel of SUTVA, which is a submodel of simple interference, which is itself a submodel of arbitrary neighborhood interference.
In general, Proposition~\ref{prop:submodel-refinement} shows that exposure-mapping submodels can be understood in terms of partition refinements.




\section{Hypothesis Testing Formulation} \label{sec:hypothesis-testing-formulation}

In this section, we formalize the problem of detecting network interference as a hypothesis test.
The hypothesis testing perspective has appeared throughout the literature on detecting interference \citeflag{}.
Our formalization will place greater emphasis on the alternatives against which we would like to achieve power.

In conventional hypothesis testing, null and alternative hypotheses $H_0$ and $H_1$ contain data generating distributions.
In a design-based context, null and alternative hypothesis will consist of entire potential outcome functions $\yv : \allinterventions \to \Reals^n$.
In particular, the null and alternative hypotheses $\modelspace_0$ and $\modelspace_1$ are model spaces.
We will focus on the setting where the null is a submodel of the alternative, i.e. $\modelspace_0 \subseteq \modelspace_1$.
The question to be answered by the hypothesis test is whether $\yv \in \modelspace_0$ or $\yv \in \modelspace_1$.

In order for a statistical test to have controlled Type I and Type II errors, we need to further limit the null and alternative models $\modelspace_0$ and $\modelspace_1$.
For example, we cannot hope to construct a test which has significant power against a potential outcome function $\yv$ which is only ``just barely'' in the alternative $\modelspace_1$.
Likewise, in order for a test to have low Type I or Type II error, we must place some sort of moment restrictions on the potential outcome functions, e.g. forbidding the situation where one subject's potential outcomes are significantly larger than the potential outcomes of all other subjects.
In order to precisely define these limitations, we need to introduce additional definitions.

\subsection{Separation Functionals} \label{sec:separation-functionals}

We begin by introducing the definition of a separation functional, which may be used to reliably distinguish potential outcome functions in the null $\modelspace_0$ from those in the alternative $\modelspace_1$.

\begin{definition}
	A functional $g : \modelspace_1 \to \Reals_{\geq 0}$ is a \emph{separation functional} if it satisfies the following two conditions:
	\begin{enumerate}
		\item \textbf{Separation}: $g(\yv) = 0$ if and only if $\yv \in \modelspace_0$.
		\item \textbf{Homogeneity}: $g( \gamma \cdot \yv ) = \gamma^2 \cdot g(\yv)$ for all $\gamma \in \Reals$ and $\yv \in \modelspace_1$.
	\end{enumerate} 
\end{definition}

A separation function provides a way of quantifying how far a potential outcome function in the alternative is from the null.
The first condition stipulates that the separation functional evaluates to 0 if and only if the entire potential outcome function $\yv$ is in the null model.
The second condition stipulates that the separation functional grows quadratically in the magnitude of $\yv$.
Together, these conditions ensure that the separation functional $g$ acts as an appropriate separator between the null and alternative models.

For general hypothesis testing problems, separation functionals will need to be constructed on a case-by-case basis, depending on the structure of the null and alternative models.
In the case where the null and alternative are both exposure mapping models, then we may define a suitable separation functional as follows:
given two nested exposure mapping models $\modelspace_{\rv} \subseteq \modelspace_{\av}$, define the \emph{refinement functional} $g : \modelspace_{\av} \to \Reals_{\geq 0}$ as
\[
g(\yv) = \frac{1}{n} \sum_{i=1}^n \sum_{R \in \rho_i} \sup \setb[\Big]{ \paren[\big]{ \alpha_{i,A} - \alpha_{i,A'} }^2 : A, A' \in \rho(R) }
\enspace.
\]
Consider a subject $i \in [n]$ and its coarser partition $\rho_i $ and finer partition $\alpha_i$, corresponding to the null $\modelspace_0$ and alternative $\modelspace_1$, respectively.
If one of the elements $R \in \rho_i$ is refined into at least two sets $A$ and $A'$, then the refinement functional reports the maximal difference in outcomes on all such refining sets, i.e. $\paren{ \alpha_{i,A} - \alpha_{i,A'} }^2$.
Note that this difference becomes larger if the two outcomes $\alpha_{i,A}$ and $\alpha_{i,A'}$ increase in magnitude.
These differences are summed over all partitions $R \in \rho_i$ and averaged across all subjects $i \in [n]$.
The following proposition demonstrates that the refinement functional is indeed a separation functional.

\begin{proposition} \label{prop:exposure-model-separation}
	The refinement functional $g$ defined above is a separation functional with respect to the nested exposure mapping models $\modelspace_{\rv} \subseteq \modelspace_{\av}$.
\end{proposition}

In Section~\placeholder, we construct a separation functional to distinguish the linear-in-means model from the SUTVA model.

\subsection{Moment Conditions} \label{sec:moment-conditions}

In design-based inference, it is often common to place moment assumptions on the potential outcome functions \citeflag{examples}.
Even simple effect estimators require bounded second moments in order to ensure consistency.
Such moment conditions on potential outcome functions $\yv$ in design-based setting are analogous to moment conditions on random outcomes in super-population settings.

A potential outcome function $\yv$ is said to be \emph{$C$-uniformly bounded} for $C > 0$ if
\[
\abs[\big]{ y_i(\zv) } \leq C 
\quad
\text{for all } \zv \in \Omega, i \in [n]
\enspace.
\]
Uniform boundedness is the strongest moment assumption considered in the literature, e.g. stronger than bounded second or fourth moments.
In this paper, our goal is to provide impossibility results: if statistical testing is impossible under uniform boundedness, then this implies impossibility for less restrictive moment conditions.

\textbf{Triangular Asymptotics}: 
While our main results are finite-sample in nature, we will often interpret them in an asymptotic context.
Keeping in convention with the design-based literature, we consider triangular array asymptotics where there is a sequence of experiments indexed by the sample size $n \in \Naturals$.
Each experiment in the sequence has its own potential outcome function $\yv^{(n)}$, model spaces $\modelspace_1^{(n)}$, $\modelspace_0^{(n)}$, and network $G^{(n)}$, although we suppress the dependence on $n$ for notational clarity.
All limiting statements are understood to be taken with respect to such an asymptotic sequence.

\subsection{Minimax Testing Error} \label{sec:formal-minimax-testing-error}

With the separation functional and moment conditions, we are now ready to define the restricted set of functions on which we hope to achieve low Type I and Type II error.
Given $C, \delta > 0$, we define the \emph{restricted null} and \emph{restricted alternative} models as
\begin{align*}
	\modelspace_0(C) &= \setb[\Big]{ \yv \in \modelspace_0 :
			\yv \textrm{ is $C$-uniformly bounded} 
			} \\
	\modelspace_1(C, \delta) &=  \setb[\Big]{ \yv \in \modelspace_1 :
			\yv \textrm{ is $C$-uniformly bounded and } 
			g(\yv) \geq \delta }
\end{align*}
A \emph{statistical test} is a measurable function $\phi : \allinterventions \times \Reals^n \to \setb{0,1}$ which takes as input the intervention $\zv$ and observed outcomes $\yv(\zv)$ and returns either $0$ or $1$ which corresponds to the null or alternative, respectively.
Given $C, \delta > 0$, we define the \emph{minimax testing error} as
\[
\risk(C, \delta) = \inf_{\substack{ \textrm{tests } \phi \\ \textrm{designs } \design }}
\braces[\Bigg]{
\sup_{\yv \in \modelspace_0(C)} \Esub[\Big]{\zv \sim \design}{ \phi( \zv, \yv(\zv) ) }
+ \sup_{\yv \in \modelspace_1(C, \delta)} \Esub[\Big]{\zv \sim \design}{ 1- \phi( \zv, \yv(\zv) ) }
}
\enspace.
\]
The minimax testing error characterizes the difficulty of the testing problem.
Note that for any potential outcome function in the null $\yv \in \modelspace_0$, the quantity $\Esub[\Big]{\zv \sim \design}{ \phi( \zv, \yv(\zv) ) }$ is the Type I error of the test $\phi$ under design $\design$.
Likewise, $\Esub[\Big]{\zv \sim \design}{ 1- \phi( \zv, \yv(\zv) ) }$ is the Type II error for a potential outcome function in the alternative, $\yv \in \modelspace_1$.
Thus, the quantity inside the inf is the sum of the worst-case Type I error and worst-case Type II error for a particular test $\phi$ and experimental design $\design$.
The minimax testing error takes into account the best choice of experimental design $\design$ and statistical test $\phi$ which minimize this error.

The quantities $C$ and $\delta$ determine the difficulty of the testing problem.
For example, the testing problem is easier for larger $\delta$, because the restrictive alternative model becomes even more well-separated from the null model.
This is formalized in the following proposition:

\begin{proposition} \label{prop:relation-of-minimax-and-quantities}
	If $C' \leq C$ and $\delta' \geq \delta$ then $\risk(C', \delta') \leq R(C, \delta)$.
\end{proposition}

The following definitions provide a distinction between testing problems which are easy and hard.
We write the risk with a subscript $n$ to reflect the dependence on the sample size.

\begin{definition} \label{def:good-test}
	A testing problem is \emph{uniformly decidable} if $\lim_{n \to \infty} \risk_n(C,\delta) \to 0$ for all $C , \delta > 0$.
	If an experimental design $\design$ and statistical test $\phi$ have risk converging to zero, they are called \emph{uniformly consistent}.
\end{definition}

\begin{definition} \label{def:impossible-test}
	A testing problem is \emph{impossible} if $R(C, \delta) = 1$ for all $C , \delta > 0$ such that $\modelspace_0(C, \delta) \neq \emptyset$.
\end{definition}

If a problem is uniformly decidable, then the Type I and Type II error can be driven to zero with enough data.
On the other hand, if a testing problem is impossible then any testing procedure will be unable to convince the experimenter whether $\yv \in \modelspace_0$ or $\yv \in \modelspace_1$.
Importantly, this is true even when we consider alternatives which are maximally far from the null, impose strong moment conditions, and have a large amount of data.
Note that $1$ is the largest possible value of minimax-testing error which is attained by a variety of trivial tests, e.g. flipping an coin independently of the observed data to decide whether to accept or reject the null.
For this reason, showing that a test is impossible is a strong negative result: its worst-case Type I and Type II error is no better than trivial tests which do not observe any data.
